Multi-Cue Adaptive Emotion Recognition Network

Expressing and identifying emotions through facial and physical expressions is a significant part of social interaction. Emotion recognition is an essential task in computer vision due to its various applications and mainly for allowing a more natural interaction between humans and machines. The common approaches for emotion recognition focus on analyzing facial expressions and requires the automatic localization of the face in the image. Although these methods can correctly classify emotion in controlled scenarios, such techniques are limited when dealing with unconstrained daily interactions. We propose a new deep learning approach for emotion recognition based on adaptive multi-cues that extract information from context and body poses, which humans commonly use in social interaction and communication. We compare the proposed approach with the state-of-art approaches in the CAER-S dataset, evaluating different components in a pipeline that reached an accuracy of 89.30%

==> images/attention_maps.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{images/attention_maps.png}
	\caption{\textmd{Visualization of the attention maps for CAER-Net-S.}}
	\label{fig:attention_maps}
\end{figure}

==> images/caer_face_sizes.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{images/caer_face_sizes.png}
	\caption{\textmd{Example of two different facial crops. Face \textbf{(a)} is the facial crop of an example from the "surprise" subset on the "train" task and has the highest resolution of the facial crops with \(422\times329\) pixels, while face \textbf{(b)} is the facial crop from an example of the "sad" subset from the "train" task and its dimensions are \(82\times82\).}}
	\label{fig:caer_face_sizes}
\end{figure}

==> images/caer_negative_pose.tex <==
\begin{figure*}%[t!]
	\centering
	\includegraphics[width=\textwidth]{images/caer_negative_pose.png}
	\caption{\textmd{Visualization of two images from the "fear" subset. In \textbf{(a)}, we see a strong activation map around the scene; however, in the original image, we can notice that these regions do not contain any important information for classification. This specific case was misclassified as "neutral." In \textbf{(b)}, we see a weak activation map on the image, meaning that the context encoding stream was unable to extract any information in this case. The proposed technique correctly classified this example, mainly due to the close-up on the face. Both of these examples would benefit from a human pose encoding stream.}}
	\label{fig:caer_negative_pose}
\end{figure*}

==> images/caerpose.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{images/CAERPose.png}
	\caption{\textmd{Examples that are prejudicial for the first proposed approach for leveraging body language. Given the amount of people in the background that does not contribute to the emotion recognition task, the body language of them are actually contributing negatively to the model. }}
	\label{fig:caerpose}
\end{figure}

==> images/ckplus.tex <==
\begin{figure}%[b]
	\centering
	\includegraphics[width=\columnwidth]{images/ckplus.png}
	\caption{\textmd{An example of preprocessing for an approach based on facial expressions \cite{JAIN201969}. The image from the CK+ dataset \cite{ck} is preprocessed to remove all non-facial features, such as background and hair.}}
	\label{fig:ckplus}
\end{figure}

==> images/foo.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{example-image}
	\caption{\textmd{Será alterado por uma imagem que explica a tarefa "logo de cara". Descreve o problema e mostra os possíveis multi-cues. Será diferente que a imagem da arquitetura.}}
	\label{fig:foo}
\end{figure}
